Verified Pythagorean Composition for Adaptive Cryptographic Games: Noise Flooding in Homomorphic Encryption

Noise flooding is a standard defense against decryption attacks on approximate homomorphic encryption, but its security proof is unusually sensitive to composition. Replacing each of $q$ adaptive decryption answers with a statistically close simulation and applying an ordinary hybrid argument loses linearly in $q$. The cryptographic proof instead accumulates conditional Kullback-Leibler (KL) costs and converts to statistical distance once, giving the parameter-critical square-root loss. We machine-check this argument using Rocq and SSProve. Given any fully homomorphic encryption scheme that is approximately correct and IND-CPA secure, we formalize a reduction for every $q$-query IND-CPAD adversary and prove \[ \Pr[\mathsf{IND\text{-}CPAD}_{\mathsf{NF}}^{\mathcal A}=1] \leq \beta_{\mathsf{CPA}}(\mathcal B_{\mathcal A,q}) + \frac{\sqrt{qn}}{2\gamma}. \] where $n$ is the plaintext dimension and $\gamma$ is the flooding-width multiplier. Our proof constructs a new relational program logic over SSProve semantics. Its Pythagorean judgment composes conditional KL budgets without converting them to statistical distance, and a verified trace compiler lifts a local oracle rule to arbitrary adaptive programs with a single final conversion.

==> macros.tex <==

\newcommand{\CameraReady}{}



\theoremstyle{definition}
\theoremstyle{definition}

\newtheorem{definition}{Definition}[section]

\newaliascnt{theorem}{definition}
\newtheorem{theorem}[theorem]{Theorem}
\aliascntresetthe{theorem}

\newaliascnt{lemma}{definition}
\newtheorem{lemma}[lemma]{Lemma}
\aliascntresetthe{lemma}

\newaliascnt{corollary}{definition}
\newtheorem{corollary}[corollary]{Corollary}
\aliascntresetthe{corollary}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbZ}{\mathbb{Z}}
\newcommand{\parens}[1]{\left(#1\right)}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\dKL}{D_{\mathrm{KL}}}
\newcommand{\KL}[2]{\dKL\!\parens{#1\,\|\,#2}}
\newcommand{\DG}[2]{D_{\bbZ,#1,#2}}
\newcommand{\distr}{\mathsf{Distr}}
\newcommand{\semantic}[1]{\llbracket #1\rrbracket}
\newcommand{\csemantic}[1]{\llbracket #1\rrbracket^{\bot}}
\newcommand{\completed}[1]{\mathsf{Comp}\parens{#1}}
\newcommand{\supp}{\mathsf{supp}}
\newcommand{\TVD}{\Delta}
\newcommand{\Pyth}{\mathsf{Pyth}}
\newcommand{\AEJ}{\mathsf{AE}}
\newcommand{\WinProb}{\mathsf{WinProb}}
\newcommand{\apRHL}{\mathsf{apRHL}}
\newcommand{\KLs}{\mathsf{KLs}}
\newcommand{\code}{\mathsf{code}}
\newcommand{\kvalid}{\mathsf{keys\_valid}}
\newcommand{\tvalid}{\mathsf{table\_valid}}
\newcommand{\doubleplus}{\mathbin{+\!\!+}}
\DeclareMathOperator{\Bern}{Bern}

